Multimodal Shape Completion via IMLE

Shape completion is the problem of completing partial input shapes such as partial scans. This problem finds important applications in computer vision and robotics due to issues such as occlusion or sparsity in real-world data. However, most of the existing research related to shape completion has been focused on completing shapes by learning a one-to-one mapping which limits the diversity and creativity of the produced results. We propose a novel multimodal shape completion technique that is effectively able to learn a one-to-many mapping and generates diverse complete shapes. Our approach is based on the conditional Implicit MaximumLikelihood Estimation (IMLE) technique wherein we condition our inputs on partial 3D point clouds. We extensively evaluate our approach by comparing it to various baselines both quantitatively and qualitatively. We show that our method is superior to alternatives in terms of completeness and diversity of shapes.

==> Tables/TotalMutualDiff.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|r|r|r}
\hline
Methods        & Chair                     & Plane & Table\\\hline
pcl2pcl        & 0                         & 0   & 0                       \\
kNN-latent     & 2.84                      & 1.13  & 3.25                    \\
Multimodal-GAN & 2.56                      & 2.03   & 4.49                   \\
Ours           & \textbf{2.93}          & \textbf{2.31}\\                     \hline
\end{tabular}
\caption{Quantitative comparison(Total Mutual Difference) with existing methods for category Chair, Plane and Table}
\label{tab:totalmutual}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{l|r|r|r}
\hline
Methods        & Chair                     & Lamp & Table \\\hline

pcl2pcl        & 0.00                      & 0.00                      \\
kNN-latent     & 2.28                      & 4.18                      \\
Multimodal-GAN & 2.56                      & 3.31                      \\
Ours           & \textbf{}                      & \textbf{5.49}    
\\ \hline
\end{tabular}
\caption{Quantitative comparison(TMD) with existing methods for category Chair, Lamp, Table [PartNet]}
\label{tab:totalmutual2}
\end{table}

==> Tables/UndirectionalHausdorffDist.tex <==
\ali{Himanshu, please make the style of this second table consistent with the previous one and cold the best number.}


\begin{table}[]
\centering
\begin{tabular}{l|r|r|r}
\hline
Methods        & Chair                     & Plane & Table\\\hline

pcl2pcl        & 5.31                      & 9.71                      \\
kNN-latent     & 8.94                      & \textbf{9.54 }                     \\
Multimodal-GAN & 9.14                      & 9.59                      \\
Ours           & \textbf{8.51}                      & 9.55    
\\ \hline
\end{tabular}
\caption{Quantitative comparison(Unidirectional Hausdorff Distance) with existing methods for category Chair and Plane}
\label{tab:und-haus-dis}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{l|r|r|r}
\hline
Methods        & Chair                     & Plane & Table\\\hline

pcl2pcl        &                       &                       \\
kNN-latent     &                      &                      \\
Multimodal-GAN &                       &                       \\
Ours           &                       &     
\\ \hline
\end{tabular}
\caption{Quantitative comparison(Unidirectional Hausdorff Distance) with existing methods for category Chair, Lamp and Table[Partnet]}
\label{tab:und-haus-dis2}
\end{table}




==> Tables/unimodal2.tex <==
\begin{table}[hbt]
    
      \centering
      \begin{tabular}{l|r|r}
\hline
Methods        & Chair                     & Plane \\\hline

pcl2pcl        & 0                      & 0                     \\
VRCNet    &   0                   & 0 \\
Ours           & \textbf{2.76}                      & \textbf{5.49} 
\end{tabular}
      

\caption{}
\label{tab:uhd}
  \end{table}
  
  

==> checklist.tex <==

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
 % \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  %\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  %\item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{refer to Section \ref{sec:experiments}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{No such impacts}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNo{No theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNo{No theoretical results.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Code will be shared upon acceptance}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{refer to \ref{sec:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Numbers shared are fairly accurate}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{refer to \ref{sec:experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Existing assets are cited.}
  \item Did you mention the license of the assets?
    \answerNA{Assets used in this research carry no license/access restrictions.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Assets used in this research carry no license/access restrictions.}
    \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{No personally identifiable information in the data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNo{No crowdsourcing.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{No crowdsourcing.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{No crowdsourcing.}
\end{enumerate}
\end{enumerate}

==> overview.tex <==
\section{Overview}
\label{sec:overview}
% Here, we provide an overview of the backbone of our method Implicit Maximum Likelihood Estimation or IMLE in short.
In shape completion problem, given a partial point cloud, we want to predict a complete point cloud based on the partially observed portion. Formally, given an input $\mathbf{x}$ in an one-to-many problem setting, the goal is to learn $p(\mathbf{y}|\mathbf{x})$ where $\mathbf{y}$ is a prediction. Here, $\mathbf{x}$ is the partial point cloud and $\mathbf{y}$ is a predicted complete point cloud. Since there are many possible complete shapes that are consistent with $\mathbf{x}$, we want to generate non-deterministic predictions $p(\mathbf{y}|\mathbf{x})$ instead of a single prediction. The simplest way to generate non-deterministic predictions is to add a random code input $\mathbf{z}\sim \mathcal{N}(0,\mathbf{I})$ to a deterministic function $T_{\theta}$ where $\mathbf{y} \coloneqq T_{\theta}(\mathbf{x}, \mathbf{z})$. This is also known as an implicit generative model~\cite{mohamed2016learning}. One way to train this implicit generative model is to use conditional GAN, in this context $T_{\theta}(\mathbf{x}, \mathbf{z})$ is often known as the generator. However, the generator may fail to generate some plausible outputs due to mode collapse. Therefore, we use Implicit Maximum Likelihood Estimation (IMLE) to train the generative model which overcomes the issue of mode collapse.

Unlike GANs, IMLE does not suffer from mode collapse as it reverses the direction of how generated samples are matched to the target data: instead of making the generated samples similar to some target data, IMLE ensures that every target data has a similar sample being generated. In addition, IMLE does not require an adversarial objective which makes it easy to train. If we denote the generator as $T_\theta(·,·)$, an input point cloud as $\mathbf{x}_i$ and the corresponding ground truth as $\mathbf{y}_i$, a latent code $\mathbf{z}_{i,j}$, then IMLE would optimize the following equation:
\begin{equation}
    \min_{\theta}\mathbb{E}_{\mathbf{z}_{1,1},\ldots,\mathbf{z}_{n,m} \sim \mathcal{N}(0, \mathbf{I})}\left[\sum_{i=1}^{n}\min_{j\in \{1,\ldots,m\}}d(T_\theta(\mathbf{x}_{i},\mathbf{z}_{i,j}), \mathbf{y}_{i})\right]
\end{equation}
where $d(·, ·)$ is a distance metric and $m$ is a hyperparameter. Algorithm~\ref{alg:cimle} shows the conditional IMLE training procedure.

\begin{algorithm}
\caption{\label{alg:cimle}Conditional IMLE Training Procedure}
\begin{algorithmic}
\Require The set of inputs $\left\{ \mathbf{x}_{i}\right\} _{i=1}^{n}$ and the set of corresponding observed outputs $\left\{ \mathbf{y}_{i}\right\} _{i=1}^{n}$
\State Initialize the parameters $\theta$ of the generator $T_\theta$
\For{$p = 1$ \textbf{to} $N$}
    \State Pick a random batch $S \subseteq \{1,\ldots,n\}$
    \For{$i \in S$}
        \State Randomly generate i.i.d. $m$ latent codes 
        \State \quad$\mathbf{z}_{1},\ldots,\mathbf{z}_{m}$
        \State $\tilde{\mathbf{y}}_{i, j} \gets T_{\theta}(\mathbf{x}_{i}, \mathbf{z}_{j})\; \forall j \in [m]$
        \State $\sigma(i) \gets \arg \min_{j} d(\mathbf{y}_{i}, \tilde{\mathbf{y}}_{i, j})\;\forall j \in [m]$
    \EndFor
    \For{$q = 1$ \textbf{to} $M$}
    \State Pick a random mini-batch $\tilde{S} \subseteq S$
    \State $\theta \gets \theta - \eta \nabla_{\theta}\left(\sum_{i \in \tilde{S}}d(\mathbf{y}_{i}, \tilde{\mathbf{y}}_{i, \sigma(i)})\right) / |\widetilde{S}|$
    \EndFor
\EndFor
\State \Return $\theta$
\end{algorithmic}
\end{algorithm}


% \subsection{Implicit Maximum Likelihood Estimation (IMLE)}

% Implicit Maximum Likelihood Estimation (IMLE) is a implicit generative model training technique. Unlike GAN doesn't suffer throught the problem of mode collapse which makes it ideal for multimodal generative models. The IMLE technique is based on the idea that instead of making the generated samples similar to real samples, it tries to ensure that every real sample has a similar sample being generated. It doesn't rely on adversarial training to bring generated and real sample closer. It generates multiple samples in every run and uses nearest neighbour to search for the generated sample which is closest to real sample. 

% % More precisely, if we denote the generator parameterized by $\theta$ as $T_\theta(·)$, which takes in a random code $z_j$ and outputs
% % a sample, IMLE optimizes the following objective:
% % \begin{equation}
% %     \min_{\theta}\mathbb{E}_{\mathbf{z}_1,\ldots,\mathbf{z}_n \sim \mathcal{N}(0,\mathbf{I})} \left[ \sum_{i=1}^N \underset{j\in \{1,\ldots,m\} }{\min} d(T_\theta(\mathbf{z}_j ),\mathbf{y}_i)\right]
% % \end{equation}
% %  where $\mathbf{y}_i$ is a real data point, $d(·, ·)$ is a distance metric and $m$ is a hyperparameter. 
% %  \ali{an illustrative figure would help here}


% \subsection{Conditional IMLE}
% In~\cite{Li2020MultimodalIS}, IMLE is extended to a conditional setting for a set of distributions $\{p(\mathbf{y}\vert\mathbf{x}_i)\}_{i=1}^{n}$. If we modify the previous notation of the generator to $T_\theta(·,·)$, an input $\mathbf{x}_i$, a latent code $\mathbf{z}_{i,j}$ and the ground truth $\mathbf{y}_i$, then IMLE would optimize the following objective:
% \begin{equation}
%     \min_{\theta}\mathbb{E}_{\mathbf{z}_{1,1},\ldots,\mathbf{z}_{n,m} \sim \mathcal{N}(0, \mathbf{I})}\left[\sum_{i=1}^{n}\min_{j\in \{1,\ldots,m\}}d(T_\theta(\mathbf{x}_{i},\mathbf{z}_{i,j}), \mathbf{y}_{i})\right]
% \end{equation}
% where $d(·, ·)$ is a distance metric and $m$ is a hyperparameter. 

% no adversarial objective is required and optimize this equation -- easy to train, explain the intuition behind how the method works(use the last part in 3.1) 


